Disentangled Representations for Manipulation of Sentiment in Text

The ability to change arbitrary aspects of a text while leaving the core message intact could have a strong impact in fields like marketing and politics by enabling e.g. automatic optimization of message impact and personalized language adapted to the receiver's profile. In this paper we take a first step towards such a system by presenting an algorithm that can manipulate the sentiment of a text while preserving its semantics using disentangled representations. Validation is performed by examining trajectories in embedding space and analyzing transformed sentences for semantic preservation while expression of desired sentiment shift.

==> 04_Experiments.tex <==

\section{Experiments}
\label{ch:experiments}
This section presents the experiments performed for evaluating the model. The results of the experiments are presented in section \ref{ch:results}.


 %------------------------------------------
\subsection{Preserving semantic content during traversal}
%------------------------------------------
In order to evaluate whether the encodings from the CNN contained information about sentiment and semantics, the feature vectors for the sentences were visualized for different sentiments and topics. The subset of feature vectors, used in each experiment, was reduced from 300 to 2 dimensions using \emph{Principal component analysis} (PCA). The visualizations were made using the first two principal components. 
To assess whether the content in a sentence is preserved in the traversal, it was desirable to traverse and visualize sentences with distinct topics. The choice of topics was sentences containing either the word ``phone'' or ``move'', because such sentences would likely have little correlation in contrast to, for example, sentences containing either ``comedy'' or ``drama''. Negative sentences containing the word ``movie'' and positive sentences containing the word ''phone'' were traversed using different settings for the hyperparameters $\sigma$ and $\lambda$. The optimization of the MMD was set up with 90 positive examples and 90 negative examples for the source and target sets. The examples consisted of an equal amount of sentences containing the word ``movie'' and sentences containing the word ``phone''. The topics of the sentences were not used for the traversal but needed when visualizing the results. For the visualization, the feature vectors for the examples and the traversed feature vectors were reduced to 2 dimensions using PCA.%, similarly to the experiment described in subsection \ref{sec:enc}. 

%------------------------------------------
\subsection{Qualitative Evaluation}
\label{sec:eval_complete}
%------------------------------------------
There exists no single correct output for the manifold traversal, e.g given the negative sentence ``The food did not taste well'', both sentences ``The food was amazing'' and ``I liked the food'' are valid outputs that reverse the sentiment. Therefore, Scores and measures used for other NLP tasks, like BLEU \cite{BLUE} for machine translation, are difficult to apply to the manifold traversal. Instead we focus on qualitative evaluation. The encoding-decoding, as well as the whole model, was evaluated by generating sentences from the feature vectors $\mathbf{z}$ (representing the original sentence) and $\mathbf{z}^*$ (the traversed vector) respectively. The generated sentences were manually compared to the original. We wanted the sentence generated from $\mathbf{z}$ to closely resemble the original sentence and the sentence generated from $\mathbf{z}^*$ to have the same context, but opposite sentiment, as the original sentence.

\subsection{Training details}
When the training of the CNN did not further improve performance, the CNN weights were locked and the RNN was retrained. The sentences from the training data were run through the trained CNN to create a set of feature vectors in 300 dimensions which served as input to the RNN. The training set was partitioned into batches of 64 sentences. All sentences shorter than 30 words were padded with ``padding tokens'' to the full length. The RNN was then trained to reproduce the original sentences over 14 epochs, given the sentence representations.

The CNN and the RNN were trained on three labelled data sets containing positive and negative sentences. The first data set is the movie review sentence polarity data set v1.0\footnote{https://www.cs.cornell.edu/people/pabo/movie-review-data/} (MR), introduced by Pang and Lee \cite{Pang+Lee:05a} in 2005. MR is a well known data set for sentiment analysis and consists of 10 662 labelled movie-review sentences from the movie review site www.rottentomatoes.com. The second data set is smaller and was introduced by Kotzias et. al \cite{DBLP:conf/kdd/KotziasDFS15} in 2015. It contains 500 reviews for cell phones and accessories from Amazon, 500 reviews for restaurants from Yelp and 500 movie reviews from IMDB\footnote{https://archive.ics.uci.edu/ml/machine-learning-databases/00331/}. Both data sets have equal amounts of positive and negative sentences. The third data set is a subset of a data set\footnote{https://github.com/oscartackstrom/sentence-sentiment-data} containing product reviews from various online sources, created by Täckström et al. \cite{Tackstrom}. In this data set, only the sentences that were either positive or negative were extracted, in total 923 positive and 1 320 negative sentences.

%The model, presented in the previous section, was implemented using the programming language Python 3. The TensorFlow \cite{tensorflow2015-whitepaper} and NumPy \cite{numpy} libraries were used for building the neural networks and the SciPy \cite{scipy} library was used for optimizing the test statistic during the manifold traversal. 

The sentiment data set was randomly separated into a training set, containing 90\% of the data, and a test set, containing the remaining 10\%. The weights in the neural networks are only updated using the loss from the training set, not the test set. The training set was divided into batches of 64 sentences and the accuracy of both neural networks was evaluated on the test set periodically every 10th batch during training. The classification accuracy of the CNN was measured by simply calculating the percentage of correctly predicted positive or negative labels on the test set. 
